Do Developers Adopt Green Architectural Tactics for ML-Enabled Systems? A Mining Software Repository Study

As machine learning (ML) and artificial intelligence (AI) technologies become more widespread, concerns about their environmental impact are increasing due to the resource-intensive nature of training and inference processes. Green AI advocates for reducing computational demands while still maintaining accuracy. Although various strategies for creating sustainable ML systems have been identified, their real-world implementation is still underexplored. This paper addresses this gap by studying 168 open-source ML projects on GitHub. It employs a novel large language model (LLM)-based mining mechanism to identify and analyze green strategies. The findings reveal the adoption of established tactics that offer significant environmental benefits. This provides practical insights for developers and paves the way for future automation of sustainable practices in ML systems.

==> Tables/size_metrics.tex <==

\begin{table*}[t]
\caption{Metrics for Different Sizes of Projects}
\centering
\footnotesize
    \begin{tabular}{|l|c|c|c|c|c|c|c|}
    \rowcolor{black}
    {\textcolor{white} {\textbf{Size}}} & {\textcolor{white} {\textbf{Number Project}}} & {\textcolor{white} {\textbf{Median Age}}} & {\textcolor{white} {\textbf{Median Stars}}} & {\textcolor{white} {\textbf{Median Size}}} & {\textcolor{white} {\textbf{Median Contributors}}} & {\textcolor{white} {\textbf{Median Forks}}} & {\textcolor{white} {\textbf{Median Commit}}} \\
    \hline
    Small & 17 & 5.7 & 157 & 244 & 3 & 44 & 95\\
    \hline
    Medium & 102 & 6.25 & 630 & 16789.5 & 9 & 131.5 & 577\\
    \hline
    Large & 49 & 6.6 & 563 & 248857 & 21 & 154 & 1506\\
    \hline
    \end{tabular}
\label{table:size_project_metrics}
\end{table*}
